Improving Spatio-Temporal Understanding of Particulate Matter using Low-Cost IoT Sensors

Current air pollution monitoring systems are bulky and expensive resulting in a very sparse deployment. In addition, the data from these monitoring stations may not be easily accessible. This paper focuses on studying the dense deployment based air pollution monitoring using IoT enabled low-cost sensor nodes. For this, total nine low-cost IoT nodes monitoring particulate matter (PM), which is one of the most dominant pollutants, are deployed in a small educational campus in Indian city of Hyderabad. Out of these, eight IoT nodes were developed at IIIT-H while one was bought off the shelf. A web based dashboard website is developed to easily monitor the real-time PM values. The data is collected from these nodes for more than five months. Different analyses such as correlation and spatial interpolation are done on the data to understand efficacy of dense deployment in better understanding the spatial variability and time-dependent changes to the local pollution indicators.

==> Temp.tex <==
Air pollution is one of the world’s largest environmental cause of disease and premature death [Lancet2018]. Because of air pollution, every year millions of people die and many more become seriously ill with cardiovascular and respiratory diseases. The issues are more aggravated in developing country like India, where air quality is a serious environmental health challenge with large sections of the population living in areas with high levels of air pollution \cite{Pant2019}. Therefore, it is important to develop tools for monitoring air pollution so that timely decisions can be made.


Cite \cite{Badura2018}: Evaluation of Low-Cost sensors for Air Pollution Monitoring

\textcolor{blue}{From Badura2008 \\Particulate matter (PM) is presently considered as one of the most serious air pollutants. PM could originate from natural sources (e.g., volcanic dust or desert dust particles and sea spray aerosols), but anthropogenic activities are also respon-
sible for its emission. Transport, agriculture, industrial
processes, and household fuel combustion can be considered
the main sources of that contaminant [1]. The adverse health effects of particulates are nowadays well documented. Exposure to PM is linked mainly to respiratory and cardiovascular health effects [2–5]. Moreover, the International Agency for Research on Cancer (IARC) classified particulates as carcinogenic to humans [6]. Today, information about the current air quality is avail-
able to the public through websites or mobile apps (for exam
ple, [7]). High-quality data for such portals comes from the
monitoring stations of governmental agencies, where auto-
mated measuring systems (AMS) are used. The most com-
monly used instruments are $\beta$-ray attenuation monitors
(BAMs) and tapered element oscillating microbalances
(TEOMs). These instruments are capable of measuring daily
and hourly PM variation. However, the spatial coverage of
monitoring stations is not very dense and nowadays new
techniques are sought to improve the spatial and temporal
resolution of PM data. Technological progress leads, among
other things, to the development of miniaturized low-cost
sensor devices and makes them promising tools for air quality monitoring application [8]. The common feature of all commercial PM sensors is the principle of operation—they measure light scattered by particles carried in an air stream through a light beam. Prices of such optical sensors range from tens to hundreds of US dollars, because they are generally cheap to manufacture. In addition, PM sensors are easy to use and in many cases ready to connect to microcomputers. Because of this, they are often adopted for use by citizen scientists [9, 11, 12]. Another advantage is low power consumption.
} 


%abstract = {Air quality remains a significant environmental health challenge in India, and large sections of the population live in areas with poor ambient air quality. This article presents a summary of the regulatory monitoring landscape in India, and includes a discussion on measurement methods and other available government data on air pollution. Coarse particulate matter (PM10) concentration data from the national regulatory monitoring network for 12 years (2004-2015) were systematically analyzed to determine broad trends. Less than 1% of all PM10 measurements (11 out of 4789) were found to meet the annual average WHO Air Quality Guideline (20 μg/m3), while 19% of the locations were in compliance with the Indian air quality standards for PM10 (60 μg/m3). Further efforts are necessary to improve measurement coverage and quality including the use of hybrid monitoring systems, harmonized approaches for sampling and data analysis, and easier data accessibility.},

Traditionally, pollution monitoring is done using stationary monitoring systems which are highly reliable, accurate and able to measure a wide range of pollutants. However, these are expensive, large and bulky, which leads to sparse deployment. This in turn leads to low spatio-temporal resolution which is not sufficient to understand the effect of pollution on the health of the citizens. Currently the pollution data is collected at few monitoring stations while the predictions of pollution levels at the locations without monitoring stations are obtained through air quality models or estimations [Barvo2012]. However, the data from the air quality models lack cross-validation and veriﬁcation. The low-cost portable ambient sensors provide a huge opportunity in increasing the spatio-temporal resolution of the air pollution information and are even able to verify, fine-tune or improve the existing ambient air quality models Previously, there have been lot of work on sensor networks for air pollution monitoring. For example, a good survey of WSN based air pollution experiments and practices has been carried out in [Yi2015]. The concepts have been extended to IoT networks in the recent times where all kinds of sensors are connected to the internet. However, most of these ideas are on conceptual level and there is dearth of actual large-scale sensor deployment and measurements, which is the focus of this paper.

Cite \cite{Tagle2020}: Air Pollution Monitoring in Chile

Cite \cite{Genikomsakis2018}: Development and On-Field Testing of Low-Cost Portable System for Monitoring PM2.5 Concentrations

Cite \cite{Pant2019}: Monitoring particulate matter in India: recent trends and future outlook



Cite Hyderabad pollution paper





The website developed for displaying the real-time air pollution is hosted at the address  \url{https:/spcrc.iiit.ac.in/air/}. The webpage is designed such that the data is fetched from ThingSpeak and is displayed on an opensource  map \emph{OpenStreetMap} \cite{OpenStreetMap}. The front-end of the webpage is designed in hyper text markup language (html) and back-end is designed in Javascript. For displaying the data on the map, we need to create the map from OpenStreetMap server and fecth the data from ThingSpeak. To get the map data, we used Javascript library \emph{Leaflet} [citation]. %which provides several  functions that can be used on map.
%To fetch the data from ThingSpeak and create the map, javascript is used as it is supported by all the browsers. 
%Javascript also has different libraries for different tasks. %There are two types of information that we need to fetch. First is the map and second is the data from ThingSpeak. 
For this, asynchronous javascript and XML (AJAX), which is a javascript library, is used, which allows us to get data from the map website and ThingSpeak API using the GET function.  

Fig. \ref{Website} shows the process flow of the website. First, the map is generated and markers are put using basic leaflet plugins and it gets the 

First we generate the map \textcolor{red}{What does this mean??} and put the marker using basic leaflet plugins and it gets the map from open street map which is an open source world map.Then we call the api using GET function available in AJAX library. After we get the data from ThingSpeak api we average the data and determine the colour associated with the value of data. Then using leaflet functions we set the marker colour and information on the map. Then the process sleeps for 5 minutes and then again calls the api and repeats the process.




%The website has been developed using javascript. The data is obtained from the ThingSpeak channel by using the thinkspeak API provided for each channel. Note that the ThingSpeak api provides only the recent data i.e., if we request 400 data points it will give us the latest 400 data points. Leaflet plugin was used to display data on map. Leaflet is a free to use plugin that has many other plugins that helps to perform a lot of actions with ease. For maps, OpenStreetMap, an open source open licensing world map, was used.   






%We get the Data from the ThingSpeak channel by using the api provided by them for each channel.We can edit the number of data points that we can fetch. We can upto 8000 data points from ThingSpeak. The ThingSpeak api provides only the recent data i.e., if we request 400 data points it will give us the latest 400 data points. 

%The ThingSpeak api gives us details for time of upload.temperature,humidity,pm2.5,pm10. It stores the data as an array of datapoints and each block is considered one element.

%AJAX GET protocol is used to call the API and get the data. Each AJAX call can fetch data from one channel so we make one AJAX call for each channel. Now the data that we receive may be inconsistent i.e., for a fixed amount of time, we might receive different number of data points depending on the network. So to make the data uniform we only take the data from an equal interval of time (in our case 5 minutes ) and average it. Then the AQI is calculated. The colour of the marker is set in accordance with the value of data. Then process is put to sleep for 5 minutes after that api calls are made again to get the for the latest five minutes and the process is repeated. 

